SpatialVisVR: An Immersive, Multiplexed Medical Image Viewer With Contextual Similar-Patient Search

In contemporary pathology, multiplexed immunofluorescence (mIF) and multiplex immunohistochemistry (mIHC) present both significant opportunities and challenges. These methodologies shed light on intricate tumor microenvironment interactions, emphasizing the need for intuitive visualization tools to analyze vast biological datasets effectively. As electronic health records (EHR) proliferate and physicians face increasing information overload, the integration of advanced technologies becomes imperative. SpatialVisVR emerges as a versatile VR platform tailored for comparing medical images, with adaptability for data privacy on embedded hardware. Clinicians can capture pathology slides in real-time via mobile devices, leveraging SpatialVisVR's deep learning algorithm to match and display similar mIF images. This interface supports the manipulation of up to 100 multiplexed protein channels, thereby assisting in immuno-oncology decision-making. Ultimately, SpatialVisVR aims to streamline diagnostic processes, advocating for a comprehensive and efficient approach to immuno-oncology research and treatment.

==> sections/Methods.tex <==
\section{Methods}

This section outlines how we utilized methodologies, including object detection, hardware setups, and Multimodal Pathology Image Retrieval (MPIR) integration, to enhance pathology data analysis and visualization, linking computational techniques with tangible user interactions.\\

\subsection{SpatialVisVR App}
\subsubsection{VR Application:}
We utilized VR for visualizing CODEX images as intricate 3D channel stacks. On the server-side, we implemented Flask to cache user-selected CODEX images in RAM for faster data retrieval. We created APIs to return channel names and the nth channel of specified CODEX images, enabling dynamic rendering in VR. We facilitated interactive coloring selection via APIs, where we processed user-selected channels server-side based on color and threshold parameters before sending them to VR for 3D arrangement and visualization, enhancing them with Unity shaders for better clarity and color vibrancy.

\vspace{10pt}
\subsubsection{GUI Overview:}
SpatialVisVR, designed for pathologists, focuses on a seamless user experience utilizing spatially multiplexed data to improve the diagnostic workflow, as showcased in Figure 4. The interface comprises three tailored windows serving distinct purposes in the diagnostic workflow.\\

The left window visualizes H\&E slides from edge detection of real-time captures, with an 'Update' button to initiate search in the third window and a primary viewing area for real-time image processing.\\

The central window, the primary viewer, facilitates exploration of CODEX ome.tiff images, allowing up to seven channel views at once for understanding cellular interactions. Essential UI elements include a sliding carousel for channel selection, a dropdown for accessing stored CODEX images, and a navigation bar for channel management, each channel color-coded for differentiation.\\

The right window visualizes search results for similar CODEX images to an H\&E slide, resembling the second window but displaying the five most similar CODEX images, aiding in further exploration.\\

Overall, the multi-window setup in SpatialVisVR enhances pathologists' workflow and diagnostic decision-making by providing diverse data examination, critical insights, and a more efficient diagnostic process. An overview of the interface is depicted in Fig. \ref{frames}.

\vspace{10pt}
\subsubsection{API Implementation}
We deployed a server-client model using RESTful APIs \cite{8385157} for communication between the server-side application and VR. A Flask application was set up on the server end, and Unity was used for processing API call data, with shaders enhancing data visualization. To address VR headset limitations, we shifted resource-intensive tasks to the server, improving user experience. The server, equipped with a 4TB SSD, hosted CODEX datasets, with data transfer rate limited to 200 MB for better VR responsiveness.
